ARM: Discovering Agentic Reasoning Modules for Generalizable Multi-Agent Systems

Large Language Model (LLM)-powered Multi-agent systems (MAS) have achieved state-of-the-art results on various complex reasoning tasks. Recent works have proposed techniques to automate the design of MASes, eliminating the need for manual engineering. However, these techniques perform poorly, often achieving similar or inferior performance to simple baselines. Furthermore, they require computationally expensive re-discovery of architectures for each new task domain and expensive data annotation on domains without existing labeled validation sets. A critical insight is that simple Chain of Thought (CoT) reasoning often performs competitively with these complex systems, suggesting that the fundamental reasoning unit of MASes, CoT, warrants further investigation. To this end, we present a new paradigm for automatic MAS design that pivots the focus to optimizing CoT reasoning. We introduce the Agentic Reasoning Module (ARM), an agentic generalization of CoT where each granular reasoning step is executed by a specialized reasoning module. This module is discovered through a tree search over the code space, starting from a simple CoT module and evolved using mutations informed by reflection on execution traces. The resulting ARM acts as a versatile reasoning building block which can be utilized as a direct recursive loop or as a subroutine in a learned meta-orchestrator. Our approach significantly outperforms both manually designed MASes and state-of-the-art automatic MAS design methods. Crucially, MASes built with ARM exhibit superb generalization, maintaining high performance across different foundation models and task domains without further optimization.

==> latex/0_Abstract.tex <==
\section{Abstract ([Shiva])}


==> latex/2_RelatedWork.tex <==
\section{Related Works}

Discuss single agent systems such as ReAct have shown to be effective. 
Then discuss papers on multi-agent systems (MAS) mentioning how they have outperformed single-agent systems on complex reasoning and planning tasks (cite a few papers here). Single agentic systems have also made a lot of progress with tool usage and other strategies. However, they have been developed for narrow tasks such as tool based search retrieval and answering. 
Then discuss how their components are heterogeneous in nature i.e., each agent has a specialized, tuned role which are different in nature and are connected in a complex topology. 
Contrary to single agent systems, our ARM approach consist multi-agent module which is applied as the repeating, basic building block. Further, ARM based MAS are also substantially more generalizable, versatile, and can be extended to any reasoning or planning tasks.


Discuss the important issue that simple operators such as CoT, multi-agent debate, and CoT-SC have shown to perform on par with these complex MAS systems.  
Discuss the issue that the foundation models have developed stronger over time, abstract level of reasoning guidance by CoT is sufficient for them. 
Discuss ADAS, Aflow, FlowReasoner, etc MAS approaches that they are tuned for a specific domain. But with recent frontier models, simple CoT and other simple operators, reasoning baseline outperforms majority of these MAS systems (as shown in our result tables in the following sections). 
Thus, more and more efforts are needed to further enhance reasoning blocks or steps in basic reasoning approaches like CoT.

==> latex/3_Approach.tex <==
\section{ARM}
We introduce the \textbf{Agentic Reasoning Module (ARM)}, a self-contained, code-based multi agentic system designed to execute a single, granular step within a complex reasoning process. ARM is conceived as a structured, agentic replacement for a single step in a Chain of Thought (CoT) sequence. While standard CoT prompts an LLM to generate the next reasoning step via naive, monolithic textual generation, an ARM employs an internal multi-agent system (MAS) to produce reasoning steps with greater structure and control. 

Following prior work, \cite{hao2023reasoning, zhang2024agentflow}, we define the multi-agentic system as a programming module - a self contained python function block, while allowing for structured control flow and access to essential APIs such as calling an external LLM, structuring the role and the prompt, and input/output format expectations. Functionally, an ARM accepts the initial problem statement and prior reasoning steps as input, and continues the reasoning until the next logical step in the solution.

\subsection{Formal Description}

Let $\mcD$ be the distribution over problem-solution pairs $(\mcQ, \mcA)$. A complete solution $\mcA$ is composed of an ordered sequence of reasoning steps $[p_1, p_2...,p_N]$ where each $p_i\in \mcP$, the space of all possible reasoning steps. We decompose the entire reasoning process into two distinct, complementary components: a \textbf{step-generator module} $(m\in\mcM)$ and a higher-level \textbf{Meta-Policy} $(\pi\in\Pi)$.
\begin{itemize}
    \item \textbf{Step Generator Module} is a function $m\in\mcQ\times\mcP^*\to\mcP$ that performs a single granular step of reasoning. It takes question $q\in\mcQ$ and the sequence of previous reasoning steps $p_{in}\in\mcP^*$ as input, and returns the next logical step $p_{out}\in\mcP$. 
    \item \textbf{Meta Policy} is a higher order function, $\pi\in\Pi:\mcQ\times\mcM\to\mcA$, that defines the overarching strategy for solving a problem. It takes a question $q$ and a specific step-generator module $m$ as inputs, orchestrates the module $m$'s execution, and returns a final solution $a\in \mcA$.  One straight-forward way to implement the meta-policy is $\pi_{Rec}^{m}$ which applies $m$ recursively until a final answer is reached.
\end{itemize}

Within in this framework, CoT can be understood as a specific pairing of  the simplest step generator and recursive meta policy, $A_{CoT}=\lambda q: \pi_{Rec}(q, m_{CoT})$

\subsection{Methodology}
We propose a dual-pronged approach to automate the discovery of high-performance agentic systems. Our method independently optimizes two key components: (1) the \textbf{step generator module} ($m \in \mcM$), which forms the core reasoning engine, and (2) the \textbf{meta-policy} ($\pi \in \Pi$), which dictates the high-level strategy for orchestrating these modules.

\subsubsection{Optimizing the Step Generator Module}
Our primary goal is to discover a step generator module, $m^*$, that is a superior, general-purpose replacement for the simple text-continuation step in CoT. We formalize a single step of reasoning as an update function, $U_{m,q}$, which takes the current reasoning history $h$ and appends the next step generated by module $m$:
$$ U_{m,q}(h) = h \cdot [m(q,h)] $$
where $\cdot$ denotes the list concatenation operator.

A full, multi-step reasoning trace generated by recursively applying this module is denoted by $\pi_{Rec}(q, m)$. If a solution requires $n$ steps, this can be expressed as the $n$-fold composition of the update function starting from an empty history, $\emptyset$:
$$ \pi_{Rec}(q, m) = U_{m,q}^n(\emptyset) = \underbrace{(U_{m,q} \circ \dots \circ U_{m,q})}_{n \text{ times}}(\emptyset) $$

Ideally, we would find the optimal module $m^*$ by maximizing the expected reward $\mathcal{R}$ over the entire recursive rollout:
$$ m^* = \underset{m\in \mcM}{\text{argmax}} \quad \E_{(q,a)\sim \mathcal{D}}\left[\mathcal{R}\left(\pi_{Rec}\left(q, m\right), a\right)\right] \label{eq:ideal_obj} $$
However, optimizing this objective directly is often intractable for two primary reasons:
\begin{itemize}
    \item \textbf{Difficult Credit Assignment:} The reward is observed only at the end of a long sequence of applications of $m$. This makes it difficult to attribute success or failure to any single step, posing a significant challenge for the search or learning algorithm.
    \item \textbf{Unconstrained Search Space:} The space of possible agentic modules $\mcM$ is vast. Without any constraints, the search is inefficient and unlikely to discover coherent, step-by-step reasoning procedures.
\end{itemize}

To overcome these challenges, we introduce a practical \textbf{scaffolded surrogate objective}. Instead of optimizing $m$ over a full, self-referential rollout, we optimize it within the context of a fixed, stable reasoning chain provided by the baseline $m_{CoT}$. Specifically, we replace a small, contiguous block of $l$ steps within an $n$-step CoT trace with our candidate module $m$. The optimization problem then becomes:
$$ m^* = \underset{m\in \mcM}{\text{argmax}} \quad \E_{(q,a)\sim \mathcal{D}}\left[\mathcal{R}\left(U_{m_{CoT},q}^i \circ U_{m,q}^l \circ U_{m_{CoT},q}^{n-l-i}(\emptyset), a\right)\right] $$
where $n = |\pi_{Rec}(q, m_{CoT})|$ is the length of the reference CoT trace, and the starting index $i$ is chosen randomly from $[0, n-l]$.

This formulation provides two key benefits. First, it isolates the effect of $m$ to a small window, making credit assignment direct and effective. Second, the surrounding CoT context provides a powerful \textbf{inductive bias}, constraining the search to modules that behave like effective, atomic reasoning steps. In practice, we find $l=3$ to be optimal, as it is long enough to expose the module $m$ to critical compositional patterns—$(U_{m_{CoT}, q} \circ U_{m,q})$, $(U_{m,q} \circ U_{m,q})$, and $(U_{m,q} \circ U_{m_{CoT},q})$—while keeping the optimization tractable.



\subsubsection{Discovering the Meta-Policy}
While an optimized step generator $m^*$ significantly improves reasoning, the meta-policy $\pi$ governing its deployment is equally critical. A simple recursive application, $\pi_{Rec}$, is effective but may not represent the optimal strategy. For instance, complex problems may benefit from parallel rollouts, self-correction loops, or other advanced schemes.

Directly searching for an optimal meta-policy $\pi^*$ using the powerful $m^*$ module is computationally prohibitive. Since each step generated by $m^*$ involves an entire internal multi-agent system, the cost of a single rollout is magnified, making large-scale exploration of the policy space $\Pi$ intractable. To overcome this challenge, we again leverage the simple CoT step generator, $m_{CoT}$, as a fast and efficient surrogate for $m^*$. We hypothesize that a meta-policy that is effective at orchestrating the simple, atomic steps of $m_{CoT}$ will generalize to the more complex, but functionally analogous, steps of $m^*$. This zero-shot transfer assumption is grounded in our step-generator optimization process (Section 3.2.1), which explicitly scaffolds $m^*$ around $m_{CoT}$ to ensure it preserves the fundamental dynamics of a sequential reasoner. 

\textcolor{red}{Bohan to fill this more.}

\subsection{Reflection Guided Search}
We optimize both the step generator $m$ and the meta-policy $\pi$ independently using a unified evolutionary search algorithm that searches the programmatic space of valid Python modules. The search history is maintained in tree, where nodes represent the specific program, and edges represent the mutations proposed by the reflection agent. The root of each tree is initialized with the baseline program, i.e., $m_{CoT}$ for the step generator and $\pi_{Rec}$ for the meta policy. 

The search iteratively performs three steps:
\begin{enumerate}
    \item \textbf{Selection:} A parent node is selected from the current tree of programs $\mathcal{T}$ using the UCB algorithm to balance exploitation and exploration: $$k = \underset{u \in \mathcal{T}}{\text{argmax}} \left( \bar{\mathcal{R}}(u) + C \sqrt{\frac{\ln T}{N_i}} \right)$$
where $\bar{\mathcal{R}}(i)$ is the node's empirical reward on the train set, T is the total number of expansions, and $N_i$ is the visit count for the node $u$.
    \item \textbf{Expansion:} A new child program is generated by the \textbf{reviewer agent}, an LLM based agent that reflects on the parent program's execution traces, correctness, and mutation history to propose targeted code modification. The prompts for the step generator and the meta agent tree expansion are given in the appendix. 
    \item \textbf{Evaluation}: The new program is evaluated against a labeled question-answer training dataset to obtain the average reward $\bar{\mathcal{R}}$  for the node, i.e. $\bar{\mathcal{R}}_{m}$ for the step generator and $\bar{\mathcal{R}}_{\pi}$ for the meta policy. The evaluation function for the step generator $m$ is the scaffolded objective (Section-2.2.1) where the module is evaluated within a $m_{CoT}$ context. For the meta policy $\pi$, we evaluate it's performance on a full problem rollout using $m_{CoT}$ as a computationally efficient surrogate for the step generator.
\end{enumerate}

\subsubsection{Reviewer Agent}
The reviewer agent is a crucial, two step process that drives the evolutionary search and returns a new Python module candidate node. It consists of two LLM based components: a \textbf{Critic}, and a \textbf{Designer}  to analyze the performance and propose targeted improvements. 

The Critic agent acts an an expert AI system reviewer. It receives the execution traces from both the current and previous version of the module (e.g. a step generator or meta-policy) and performs a pairwise comparison. The critic's primary objective is to analyze how the design modification impacts performance, and provide insights  grounded in the provided execution data. These insights inform the subsequent evolution of the module. Then, a Designer agent acts as the mutation operator. It receives the module to evolve, its performance history, and the critic's analysis to propose a single, novel code modification aimed at improving performance. This agent operates within a strict programmatic framework, generating a complete Python class that adheres to predefined API and structural constraints. The full prompts for the Critic and the Designer are provided in the Appendix-.

\begin{algorithm}[h!]
\caption{Reflection-Guided Search}
\label{alg:rets}
\begin{algorithmic}[1]
\State \textbf{Input:} Initial program $p_{root}$ (e.g., $m_{CoT}$ or $\pi_{Rec}$), evaluation function $\textsc{Evaluate}(\cdot)$, total iterations $K$, exploration constant $C$.
\State \textbf{Initialize:}
\State Tree $\mathcal{T}$ with a single node for $p_{root}$.
\State $p_{root}.\bar{\mathcal{R}} \leftarrow \textsc{Evaluate}(p_{root})$ \Comment{Evaluate the baseline program on a validation batch}
\State $p_{root}.N \leftarrow 1$ \Comment{Initialize visit count for the root}

\For{$t=1$ \textbf{to} $K$}
    \State \Comment{\textit{1. Select a parent program to mutate}}
    \State $p_{parent} \leftarrow \underset{p_i \in \mathcal{T}}{\text{argmax}} \left( p_i.\bar{\mathcal{R}} + C \sqrt{\frac{\ln t}{p_i.N}} \right)$
    
    \State \Comment{\textit{2. Expand the tree via reflection}}
    \State traces $\leftarrow$ \textsc{Execute}($p_{parent}$) \Comment{Collect execution traces}
    \State history $\leftarrow$ \textsc{GetMutationHistory}($p_{parent}$)
    \State $p_{new} \leftarrow \textsc{ReviewerAgent}(p_{parent}, \text{traces}, \text{history})$
    
    \State \Comment{\textit{3. Evaluate the new program}}
    \State $p_{new}.\bar{\mathcal{R}} \leftarrow \textsc{Evaluate}(p_{new})$
    \State $p_{new}.N \leftarrow 1$
    
    \State \Comment{\textit{4. Update tree and statistics}}
    \State $\mathcal{T}.\textsc{AddChild}(p_{parent}, p_{new})$
    \State $p_{parent}.N \leftarrow p_{parent}.N + 1$
\EndFor
\State
\State \textbf{return} $\underset{p_i \in \mathcal{T}}{\text{argmax}} \ (p_i.\bar{\mathcal{R}})$ \Comment{Return the program with the highest empirical reward}
\end{algorithmic}
\end{algorithm}




==> latex/5_DUMMY.tex <==
\subsection{Methodology}
We propose a dual-pronged approach to automate the discovery of high-performance agentic systems. Our method independently optimizes two key components: (1) the \textbf{step generator module} ($m \in \mcM$), which forms the core reasoning engine, and (2) the \textbf{meta-policy} ($\pi \in \Pi$), which dictates the high-level strategy for orchestrating these modules.

\subsubsection{Optimizing the Step Generator Module}
Our primary goal is to discover a step generator module, $m^*$, that is a superior, general-purpose replacement for the simple text-continuation step in CoT. We formalize a single step of reasoning as an update function, $U_{m,q}$, which takes the current reasoning history $h$ and appends the next step generated by module $m$:
$$ U_{m,q}(h) = h \cdot [m(q,h)] $$
where $\cdot$ denotes the list concatenation operator.

A full, multi-step reasoning trace generated by recursively applying this module is denoted by $\pi_{Rec}(q, m)$. If a solution requires $n$ steps, this can be expressed as the $n$-fold composition of the update function starting from an empty history, $\emptyset$:
$$ \pi_{Rec}(q, m) = U_{m,q}^n(\emptyset) = \underbrace{(U_{m,q} \circ \dots \circ U_{m,q})}_{n \text{ times}}(\emptyset) $$

Ideally, we would find the optimal module $m^*$ by maximizing the expected reward $\mathcal{R}$ over the entire recursive rollout:
$$ m^* = \underset{m\in \mcM}{\text{argmax}} \quad \E_{(q,a)\sim \mathcal{D}}\left[\mathcal{R}\left(\pi_{Rec}\left(q, m\right), a\right)\right] \label{eq:ideal_obj} $$
However, optimizing this objective directly is often intractable for two primary reasons:
\begin{itemize}
    \item \textbf{Difficult Credit Assignment:} The reward is observed only at the end of a long sequence of applications of $m$. This makes it difficult to attribute success or failure to any single step, posing a significant challenge for the search or learning algorithm.
    \item \textbf{Unconstrained Search Space:} The space of possible agentic modules $\mcM$ is vast. Without any constraints, the search is inefficient and unlikely to discover coherent, step-by-step reasoning procedures.
\end{itemize}

To overcome these challenges, we introduce a practical \textbf{scaffolded surrogate objective}. Instead of optimizing $m$ over a full, self-referential rollout, we optimize it within the context of a fixed, stable reasoning chain provided by the baseline $m_{CoT}$. Specifically, we replace a small, contiguous block of $l$ steps within an $n$-step CoT trace with our candidate module $m$. The optimization problem then becomes:
$$ m^* = \underset{m\in \mcM}{\text{argmax}} \quad \E_{(q,a)\sim \mathcal{D}}\left[\mathcal{R}\left(U_{m_{CoT},q}^i \circ U_{m,q}^l \circ U_{m_{CoT},q}^{n-l-i}(\emptyset), a\right)\right] $$
where $n = |\pi_{Rec}(q, m_{CoT})|$ is the length of the reference CoT trace, and the starting index $i$ is chosen randomly from $[0, n-l]$.

This formulation provides two key benefits. First, it isolates the effect of $m$ to a small window, making credit assignment direct and effective. Second, the surrounding CoT context provides a powerful \textbf{inductive bias}, constraining the search to modules that behave like effective, atomic reasoning steps. In practice, we find $l=3$ to be optimal, as it is long enough to expose the module $m$ to critical compositional patterns—$(U_{m_{CoT}, q} \circ U_{m,q})$, $(U_{m,q} \circ U_{m,q})$, and $(U_{m,q} \circ U_{m_{CoT},q})$—while keeping the optimization tractable.


\subsubsection{Discovering the Meta-Policy}
While an optimized step generator $m^*$ improves the quality of individual reasoning steps, the meta-policy $\pi$ that orchestrates these steps is equally critical for solving complex problems. A simple recursive application, $\pi_{Rec}$, is a strong baseline but is often suboptimal. More sophisticated strategies involving parallel rollouts, self-correction loops, or dynamic resource allocation can yield superior performance.

Directly searching for an optimal meta-policy $\pi^*$ using the powerful $m^*$ module is computationally prohibitive. Since each step generated by $m^*$ involves an entire internal multi-agent system, the cost of a single rollout is magnified, making large-scale exploration of the policy space $\Pi$ intractable.

To surmount this challenge, we again leverage the simple CoT step generator, $m_{CoT}$, as a fast and efficient **surrogate** for $m^*$. We hypothesize that a meta-policy that is effective at orchestrating the simple, atomic steps of $m_{CoT}$ will generalize to the more complex, but functionally analogous, steps of $m^*$. This zero-shot transfer assumption is grounded in our step-generator optimization process (Section 2.2.1), which explicitly scaffolds $m^*$ around $m_{CoT}$ to ensure it preserves the fundamental dynamics of a sequential reasoner.
**************

\subsection{Reflection-Guided Evolutionary Tree Search}
To discover the optimal Step Generator ($m^*$) and Meta-Policy ($\pi^*$), we employ the same core search algorithm for both. The method is a form of evolutionary search that explores a complex programmatic space by organizing the search history into a tree. This approach allows us to efficiently navigate the vast space of possible programs while intelligently guiding the search with a reflection mechanism.

\subsubsection{Programmatic Search Space and Tree Representation}
Our search operates over a discrete and programmatic space where each element is a self-contained, executable module. For the step generator, this is a Python function implementing the logic for a single reasoning step. For the meta-policy, it is a higher-level script that orchestrates calls to a step generator. These programs are not limited to simple sequential logic; they can include complex control flow (e.g., conditionals, loops), invoke external tools, manage intermediate states, and call LLMs with different roles and instructions, forming a rich space of possible agentic behaviors.

We represent the evolutionary lineage and relationships of these programs using a tree structure:
\begin{itemize}
    \item \textbf{Nodes:} Each node in the tree corresponds to a unique, version-controlled program. A node stores the complete source code of the program, its empirically measured performance score ($\bar{\mathcal{R}}$), and metadata such as the reflective analysis from the reviewer agent that led to its creation.
    \item \textbf{Root:} The root of the tree represents the initial baseline program—either the simple $m_{CoT}$ for step generator search or the recursive $\pi_{Rec}$ for meta-policy search. This serves as the primordial seed for evolution.
    \item \textbf{Edges:} A directed edge from a parent node to a child node signifies an evolutionary step. It represents a single, targeted mutation applied by the reviewer agent to transform the parent's code into the child's. The tree, therefore, maps the complete evolutionary history of every candidate program.
\end{itemize}
This explicit tree representation allows the search to maintain a comprehensive history of exploration, enabling the reviewer agent to make more informed decisions by analyzing entire branches of successful or failed mutation paths.

\subsubsection{The Evolutionary Search Loop}
The search proceeds iteratively, repeatedly applying three phases: Selection, Expansion, and Evaluation.

\paragraph{1. Selection}
In each iteration of the search, we select an existing node in the tree to serve as the basis for a new mutation. This choice is critical, as it balances **exploiting** programs we know are good with **exploring** the potential of others. We use the Upper Confidence Bound (UCB) formula to select a node $k$ from the set of all current nodes $\mathcal{K}$ in the tree:
$$ k = \underset{i \in \mathcal{K}}{\text{argmax}} \left( \bar{\mathcal{R}}(i) + C \sqrt{\frac{\ln T}{N_i}} \right) $$
Here, $\bar{\mathcal{R}}(i)$ is the known mean reward of the program at node $i$. $T$ is the total number of mutations performed so far in the search, and $N_i$ is the number of times node $i$ has been chosen as a parent for mutation. The exploration constant $C$ balances the two terms.

\paragraph{2. Expansion and Reflection}
Once a parent node (program) is selected, it is expanded by creating a new child node. This is performed by our LLM-based **"reviewer agent"**. The agent reflects on the parent program's behavior by analyzing its source code, execution traces from a sample batch, and the historical performance of previous mutations from that parent. Based on this analysis, it proposes a targeted code mutation to create a new child program.

\paragraph{3. Evaluation}
The newly created child program must be evaluated to obtain its performance score, $\bar{\mathcal{R}}$. This is the only component of our algorithm that differs between the optimization of the step generator and the meta-policy.

\subsubsection{Step Generator Evaluation}
When optimizing the step generator module $m$, its performance is measured using the **scaffolded objective function** detailed in Section 2.2.1. A candidate module $m'$ is executed for a small number of steps ($l=3$) within the stable context of a surrounding $m_{CoT}$ execution chain.

\subsubsection{Meta-Policy Evaluation}
When optimizing the meta-policy $\pi$, its performance is measured over a full problem rollout. To ensure this evaluation remains computationally tractable, we use the efficient $m_{CoT}$ module as a surrogate for the step generator throughout the rollout. The final reward of the complete trajectory serves as the policy's score.

\begin{algorithm}[h!]
\caption{Reflection-Guided Evolutionary Tree Search (RETS)}
\label{alg:rets}
\begin{algorithmic}[1]
\State \textbf{Input:} Initial program $p_{root}$ (e.g., $m_{CoT}$ or $\pi_{Rec}$), evaluation function $\textsc{Evaluate}(\cdot)$, total iterations $K$, exploration constant $C$.
\State \textbf{Initialize:}
\State Tree $\mathcal{T}$ with a single node for $p_{root}$.
\State $p_{root}.\bar{\mathcal{R}} \leftarrow \textsc{Evaluate}(p_{root})$ \Comment{Evaluate the baseline program on a validation batch}
\State $p_{root}.N \leftarrow 1$ \Comment{Initialize visit count for the root}

\For{$t=1$ \textbf{to} $K$}
    \State \Comment{\textit{1. Select a parent program to mutate}}
    \State $p_{parent} \leftarrow \underset{p_i \in \mathcal{T}}{\text{argmax}} \left( p_i.\bar{\mathcal{R}} + C \sqrt{\frac{\ln t}{p_i.N}} \right)$
    
    \State \Comment{\textit{2. Expand the tree via reflection}}
    \State traces $\leftarrow$ \textsc{Execute}($p_{parent}$) \Comment{Collect execution traces}
    \State history $\leftarrow$ \textsc{GetMutationHistory}($p_{parent}$)
    \State $p_{new} \leftarrow \textsc{ReviewerAgent}(p_{parent}, \text{traces}, \text{history})$
    
    \State \Comment{\textit{3. Evaluate the new program}}
    \State $p_{new}.\bar{\mathcal{R}} \leftarrow \textsc{Evaluate}(p_{new})$
    \State $p_{new}.N \leftarrow 1$
    
    \State \Comment{\textit{4. Update tree and statistics}}
    \State $\mathcal{T}.\textsc{AddChild}(p_{parent}, p_{new})$
    \State $p_{parent}.N \leftarrow p_{parent}.N + 1$
\EndFor
\State
\State \textbf{return} $\underset{p_i \in \mathcal{T}}{\text{argmax}} \ (p_i.\bar{\mathcal{R}})$ \Comment{Return the program with the highest empirical reward}
\end{algorithmic}
\end{algorithm}

\subsection{Analysis of the Meta Policy}
The goal of the Meta Policy is to learn a policy ($\pi_M$) which uses the subroutine $M$ as the step generator. 

The crucial challenge in learning a meta policy based on the learned step generator $m$ is the intractability of credit assignment through deep reflection of the rollout. This is because B is a complex agentic block with significantly longer rollouts compared to the base CoT. To overcome this, we propose learning the scaffold on the weaker, but easy to handle CoT block, and use it with the block B learned in the local strategy discovery phase. This trick intuitively works because B learns to operate in the context of recursive CoT calls and preserves certain dynamics of CoT such as input, output formats, granular progress etc. We present a formal analysis below. 

\subsubsection{Notation}
\textbf{Scaffold Policy ($\pi_M$)}: the meta orchestrator policy (scaffold policy) with $M$ as the partial progress sub-routine. For simplicity, let's represent CoT as sub-routine $A$ and the discovered block as $B$, i.e, $M\in\{A, B\}$.

\textbf{State space ($S$)}: state space of the scaffold policy $\pi_M$, which is typically the input question and the accumulated progress from the calls to the subroutine $M$. 

\textbf{Transition Probability $(P_M(s'|s))$}: the state transition probability of $\pi_M$. $P_A(s'|s)$ and $P_B(s'|s)$ represents the transition probability for CoT and the discovered block respectively.

\textbf{Stationary Distributions ($d_M(s)$)}: distribution of states visited by $\pi_M$ thus yeilding $d_A(s)$ and $d_B(s)$ for CoT and the block respectively. 

\textbf{Reward $(R(s, s'))$}: A valid reward function assigning partial rewards when transitioning from state $s$ to $s'$

\textbf{Value Functions $(V_A, V_B)$}: The expected cumulative reward starting from a state s and following policy $\pi_M$. We assume a discounted setting as follows:
\begin{itemize}
    \item $V_A(s)=\E_{\pi, P_A}[\sum_{t=0}^{t=\infty}\gamma^tr(s_t, s_{t+1}) | s_0=s]$
    \item $V_B(s)=\E_{\pi, P_B}[\sum_{t=0}^{t=\infty}\gamma^tr(s_t, s_{t+1}) | s_0=s]$
\end{itemize}


\subsubsection{Idealized Conditions for Off-Policy Transfer}
Our goal is to show that, on average, deploying the scaffold policy with $B$ in lieu of $A$ yields a better overall model. Formally, we want to show: $\mathbb{E}_{s \sim d_B}[V_B(s)] \geq \mathbb{E}_{s \sim d_A}[V_A(s)]$. The success of this argument rests on the following idealized conditions that our local strategy is designed to promote:

\textbf{1. Dominance over Expectation:} The expected value function of a state using B is at least as good as A, on expectation over all the states reachable by the $\pi_A$. 

$$\E_{\rs\sim d_A}[V_B(s)] \geq \E_{\rs\sim d_A}[V_A(s)]$$
\underline{Justification:} This assumption states that the meta policy $\pi_M$ trained on the subroutine $A$ will perform better when using the subroutine $B$ instead of A is central to our meta policy. This is a strong off-policy transfer claim, but one that is justified by the specific design of the local strategy block which ensures that $B$ is a \textbf{monotonically improving} and \textbf{dynamically compatible} replacement for $A$. Our claim rests on the following arguments:

\textbf{CoT scaffolding enforces Dynamics Compatibility}: 
    
The primary risk of swapping the subroutine $A$ with $B$ is the mismatch in the dynamics which renders the meta policy ineffective. However, our scaffolded training is a direct counter measure to this risk, as $b$ is not trained in isolation, but in the context and eco-system of CoT reasoning. Thus $b$ learns to:
\begin{itemize}
    \item \textbf{Accept} $c$ style inputs as block $b$ is fed the output states from applying preceding $c$ block.
    \item \textbf{Return} $c$ style outputs as the subsequent block $c$ is fed the output states from the $b$ block.
    \item \textbf{Self Interact} with itself where it gets an input state from itself and passes the output state to itself.
\end{itemize}
This forces the block to implicitly model the dynamics of the CoT block. Therefore, the transition shift $P_A\to P_B$ is not arbitrary, but a constrained shift where the fundemental rules of state progression are preserved, ensuring that $\pi_M$'s learned orchestration remains effective.
    
\textbf{B is a Monotonically Improving successor to CoT}

\textcolor{blue}{The second risk to this strategy is that B's local improvements do not translate to global gains. We argue that our reflective meta agent functions as a powerful, implicit Generalized Policy Improvement (GPI) like operator.} A frontier LLM has been pretrained on large training corpus of code, reasoning and humanity's collective knowledge. This can be conceptualize d as the LLM having an implicit access to an enormous corpus of "sub-policies" or "skills". When the meta agent performs it's deep reflective thinking, it thoroughly deconstructs and analyzes the parent policy $\pi_{M}^{(i)}$ rollout, and identifies the local code parts that succeeded, and those that failed or potentially can fail and relies on it's internal knowledge to propose an incremental modification. Thus, the creation of new policy is not an aribitrary exploration, but an inherently compositional act, drawing from the successful parts of $\pi_{M}^{(i)}$, and the superior alternatives sampled from it's implicit library of sub-policies.
    
Furthermore, our \textcolor{red}{empirical results in Table} show that this is true in practice. 

\textbf{2. Beneficial Distribution Shift:} The distribution shift from $d_A$ to $d_B$ is such that it moves the state distribution towards states with a higher value function under B.
$$\E_{\rs\sim d_B}[V_B(s)] \geq \E_{\rs\sim d_A}[V_B(s)]$$
    

\underline{Justification:} This assumption states that interaction with B leads to more beneficial states for the policy than A on expectation. This is again a straightforward consequence of the training set-up where B learns to produce better partial progress (accumulated state) than the baseline A. A superior partial progress generator would naturally guide the policy towards more promising soution trajectories.

\subsubsection{Analysis}
Under these idealized assumptions, let's compare the average expected values $\bar{V}_B = \mathbb{E}_{s \sim d_B}[V_B(s)]$ and $\bar{V}_A = \mathbb{E}_{s \sim d_A}[V_A(s)]$. 

We can decompose the difference $\bar{V}_B - \bar{V}_A$ as 
$$\bar{V}_B - \bar{V}_A = \sum_s d_B(s) V_B(s) - \sum_s d_A(s) V_A(s)$$
$$\bar{V}_B - \bar{V}_A = \underbrace{\left(\sum_s d_B(s) V_B(s) - \sum_s d_A(s) V_B(s)\right)}_{\text{Change due to distribution shift}} + \underbrace{\left(\sum_s d_A(s) V_B(s) - \sum_s d_A(s) V_A(s)\right)}_{\text{Performance gain from B}}$$

The first term represents the performance improvement when using B but the state distribution remained the same as with A. 

$$\sum_s d_A(s) V_B(s) - \sum_s d_A(s) V_A(s) = \sum_s d_A(s) [V_B(s) - V_A(s)]$$
$$= \E_{\rs\sim d_A}[V_B(s) - V_A(s)]$$

By assumption 1, this term is is $\geq 0$

Now consider the second term:
$$\sum_s d_B(s) V_B(s) - \sum_s d_A(s) V_B(s) = \E_{\rs\sim d_B}[V_B(s)] - \E_{\rs\sim d_A}[V_B(s)]$$

This is also $\geq 0$ by assumption 2, which yields the final result

$$\bar{V}_B \geq \bar{V}_A$$



==> latex/B_Theory.tex <==

\section{Theoretical Analysis}
\label{sec:apdx_theoritical_analysis}
A complete theoretical analysis of the multi-agentic system ARM powered by LLMs is intractable due to the complex, high-dimensional nature of language generation and the non-stationary of the generation process. Therefore, to build a formal intuition for the design choices in our scaffolded search for the step-generator, and the decoupled search for the meta-policy (Algorithm\ref{alg:rets}), we analyze an idealized formulation of the problem as a Markov Decision Process (MDP). This abstracts away the underlying complexities of the text generation and focuses on the dynamics of per-step error and state distribution shift. This analysis provides a formal intuition for the soundness of our proposed search objective. 


\subsection{An Idealized MDP Model of Step-wise Reasoning}
We model the reasoning process as a Markov decision process (MDP) \cite{10.5555/3312046} $\mathcal{M} = (S, A, P, R, \gamma)$:
\begin{itemize}
    \item \textbf{State Space $(S)$:} The state space $S=S_{ok}\cup S_{fail}\cup S_{done}$ is partitioned into three disjoint subsets: 
    \begin{itemize}
        \item $S_{ok}$: A state $s\in S_{ok}$ represents a partial reasoning trace ${q, p_1, ...p_k}$ that is on a valid path to a solution. 
        \item $S_{fail}$: A state $s\in S_{fail}$ has made a critical reasoning error from which recovery is not possible (including terminal states where the reasoning chain ended up on the wrong answer). This is an absorbing region.
        \item $S_{done}$: A state $s\in S_{done}$ represents a reasoning path that has successfully ended on the right answer. This is an absorbing region.
    \end{itemize}    
    \item \textbf{Action Space $(A)$}: For a fixed meta-policy $\pi_{Rec}$ that recursively generates steps until termination (such as the one used by baseline CoT or the ARM-only variant), the meta policy executes a single action at any give state $s\in S_{ok}$: i.e., invokes a step-generator module $m$ to produce the next reasoning step. Thus, the action space is a singleton $\mathcal{A}=\{\texttt{generate\_step}\}$. Hence, the choice of the module $m$ fully defines the transition dynamics of the MDP.
    \item  \textbf{Reward Function $(R)$: } A sparse reward function with $R=1$ given upon transition to a done state.
    \begin{itemize}
        \item $R(s) = 1$ if $s \in S_{done}$ and $0$ otherwise.
    \end{itemize}
    \item \textbf{Transition Dynamics (P)}: update function (see 3.2.1) $U_{m, .}$ where $m\in\mathcal{M}$ is characterized by its state-dependent error rate, $\epsilon_m(s)$, which is the probability of making a catastrophic irrecoverable error from state $s$. Additionally, we introduce For any state $s\in S$, the transition probabilities to the next state $s'$ are defined as:

    \begin{itemize}
        \item $
        P(s' | s, m) = 
\begin{cases} 
   p_{done}(s) & \text{if } s' \in S_{done} \\
   \epsilon_m(s) & \text{if } s' \in S_{fail} \\
   1 - p_{done}(s) - \epsilon_m(s) & \text{if } s' \in S_{ok}
\end{cases}
        $ 


Note that $p_{done}(s)$ is the intrinsic probability of finishing the task by transitioning into a done state from state $s$. In practice, this is when the model emits \texttt{//boxed[Correct Answer]}. This can be assumed to be a property of the task and the progress so far, rather than the generator itself. 
\end{itemize}
\item \textbf{Value Function:} The value of a state $s$ under module $m$, denoted by $V_m(s)$ is the probability of eventually reaching a success state in $S_{done}$ (thus receiving a reward) starting from $s$. 
\end{itemize}

Within in MDP framework, the ideal objective is to discover a module $m^*$, that maximizes the expected value from the initial state distribution $d_0(s)$

$$m^*=\underset{m\in\mathcal{M}}{\text{arg\, max}\,}\mathbb{E}_{s_0\sim d_0(s)}\left[V_m(s_0)\right]$$
This objective poses several major optimization challenges: 1) credit assignment problem over long sequence of steps and 2) unconstrained search space of code modules. 


\subsection{Theoretical Grounding for the Scaffolded Step-Generator Search}
\label{sec:apdx_scaffolding_step_generator_theory}

The scaffolded objective evaluates a candidate $m$ by \emph{splicing} it into a baseline rollout for a short window
$t\in\{i,\dots,i+\ell-1\}$ while keeping $m_{\text{CoT}}$ before and after:
\[
\underbrace{U^{*}_{m_{\text{CoT}}}\circ \big(\,U^\ell_{m}\,\big)\circ U^{i}_{m_{\text{CoT}}}}_{\text{“baseline–candidate–baseline”}}.
\]
Let $d_{\text{CoT},t}$ be the state distribution at step $t$ along the (unperturbed) baseline trace.
Define the single-step advantage $A_m(s)\coloneqq V_m(s)-V_{\text{CoT}}(s)$.

% \paragraph{Assumption 1 (Finite-horizon conditional stability).}
% \label{conditional_trust_region}
% Within the $l$-step scaffold window, and for states 
% $s \sim d_{\text{CoT},t}$ encountered along the baseline trace, 
% the conditional distribution over next states produced by a candidate 
% module $m$ (restricted to transitions that remain in $S_{ok}$) 
% does not diverge significantly from that of the baseline 
% $m_{\text{CoT}}$. Formally,
% \[
% \mathbb{E}_{s \sim d_{\text{CoT},t}} \Big[
% D_{\mathrm{TV}}\!\left(
% \mathcal{T}_m(\cdot \mid s, S_{ok}) \,\big\|\, 
% \mathcal{T}_{\text{CoT}}(\cdot \mid s, S_{ok})
% \right)
% \Big] \;\leq\; \beta_{ok},
% \quad \text{for each } t \in \{i,\ldots,i+l-1\},
% \]
% for some small constant $\beta_{ok} > 0$.

\begin{assumption}[Finite-horizon conditional stability]\label{ass:conditional-stability}
Within the scaffold window and for states along the baseline trace ($s\sim d_{\text{CoT},t}$),
the \emph{conditional} next-state distributions inside $\mathcal S_{ok}$ remain close:
\[
\mathbb E_{s\sim d_{\text{CoT},t}}
\Big[
D_{\mathrm{TV}}\big(T_m(\cdot\mid s, \mathcal S_{ok})\,\Vert\,T_{\text{CoT}}(\cdot\mid s, \mathcal S_{ok})\big)
\Big]\;\le\;\beta_{ok}\quad \forall t\in\{i,\dots,i+\ell-1\}.
\]
\end{assumption}
\begin{itemize}
    \item \textbf{Remark:} This constraint requires that, conditional on the trajectory staying in $S_{ok}$, the distribution over possible next states under module $m$ is close on average (in total variation distance) to the distribution under $m_{\text{CoT}}$.  

This assumption is grounded in the mechanics of the prompted LLMs. The scaffold provides a strong contextual prior (the preceding CoT steps) and acts as a powerful inductive bias, strongly constraining the module to generate a next step that is stylistically and logically consistent with the atomic reasoning style of CoT. For instance, by defining variables in the same format, using consistent LaTeX for equations, or following an established deductive pattern (e.g., '\texttt{Let x be..., then it follows that y..., therefore z...}' etc.). This incentivizes the LLM to generate a coherent and logically plausible continuation---a necessary condition for remaining in $S_{ok}$. Therefore, any ``successful'' module $m$ must, by necessity, learn to mimic the local \emph{successful} behavior of $m_{CoT}$ while minimizing the transition probability to hazard states $S_{fail}$. This is empirically supported by the examples shown in Appendix-\ref{sec:step_rollout_examples}. 

\end{itemize}

\begin{proposition}[Scaffolded objective optimizes per-step error rate]\label{prop:scaffold-advantage}
Let $w_t$ be the probability the baseline remains in $\mathcal S_{ok}$ up to step $t$.
Then for a universal constant $C>0$,
\[
V_{\text{scaffold}}(m)-V_{\text{scaffold}}(m_{\text{CoT}})
\;\ge\;
\sum_{t=i}^{i+\ell-1}\mathbb E_{s\sim d_{\text{CoT},t}}\!\big[A_m(s)\big]
\;-\; C\sum_{t=i}^{i+\ell-1} w_t\,\beta_{ok}.
\]
Moreover, under Assumption~\ref{ass:conditional-stability}, $A_m(s)$ is dominated by \emph{error-rate reduction}:
\[
A_m(s)\;\approx\;\big(\varepsilon_{\text{CoT}}(s)-\varepsilon_m(s)\big)\cdot \mathbb E_{s'\sim T_{\text{CoT}}(\cdot\mid s,\mathcal S_{ok})}\!\big[V_{\text{CoT}}(s')\big].
\]
\end{proposition}

\begin{proof}[Proof of Proposition~\ref{prop:scaffold-advantage}]
By Assumption-\ref{ass:conditional-stability}, the performance improvement within the $l$-step scaffold window is lower bounded by the cumulative advantage, minus a small penalty for the distribution shift on successful steps \cite{10.5555/645531.656005, pmlr-v37-schulman15}. 

{\small \underline{\textit{Side Note:}} For the purpose of a conservative lower bound, we treat this term
as a penalty. However, in practice such conditional distributional shift may be
beneficial: an advanced module $m$, potentially using mechanisms like self-consistency
or debate, could guide the trajectory toward higher-value states even within
$\mathcal S_{ok}$. This would add a positive contribution, but our main result does
not rely on that stronger assumption.}


% \footnote{For the purpose of a conservative lower bound, we treat this term as a penalty. However, it is worth noting that this conditional distributional shift on successful steps is, in fact, beneficial. An advanced module m, potentially incorporating mechanisms analogous to self-consistency or debate , may guide the trajectory towards higher-value states even within $S_{ok}$. This would yield a positive contribution from the distributional shift, representing an additional source of gain. We note that our main result does not rely on this stronger assumption.}. 

For a step $t$ and a baseline state $s\in\mathcal S_{ok}$, the Bellman equation with our transitions gives
\[
V_m(s)=p_{\text{done}}(s)\cdot 1 + \big(1-p_{\text{done}}(s)-\varepsilon_m(s)\big)\cdot
\mathbb E_{s'\sim T_m(\cdot\mid s,\mathcal S_{ok})}\big[V_m(s')\big].
\]
Subtract the corresponding identity for $V_{\text{CoT}}(s)$ and rearrange:
\begin{align*}
A_m(s)
&=V_m(s)-V_{\text{CoT}}(s)\\
&=\underbrace{\big(\varepsilon_{\text{CoT}}(s)-\varepsilon_m(s)\big)\,
\mathbb E_{s'\sim T_{\text{CoT}}(\cdot\mid s,\mathcal S_{ok})}\!\big[V_{\text{CoT}}(s')\big]}_{\text{error-rate reduction term}}
\\[-2mm]
&\quad +\underbrace{\big(1-p_{\text{done}}(s)-\varepsilon_m(s)\big)\,
\big(\mathbb E_{s'\sim T_m}[V_m(s')]-\mathbb E_{s'\sim T_{\text{CoT}}}[V_{\text{CoT}}(s')]\big)}_{\triangle(s)}.
\end{align*}
By Assumption~\ref{ass:conditional-stability}, the conditional distributions inside $\mathcal S_{ok}$ are close in total variation, hence (by standard TV–expectation inequalities) for some constant $C'>0$,
\[
\big|\mathbb E_{s'\sim T_m}[V_m(s')]-\mathbb E_{s'\sim T_{\text{CoT}}}[V_{\text{CoT}}(s')]\big|
\;\le\; C'\,\beta_{ok}.
\]
Since $0\le 1-p_{\text{done}}(s)-\varepsilon_m(s)\le 1$, we have $|\triangle(s)|\le C'\beta_{ok}$.
Taking expectations over $s\sim d_{\text{CoT},t}$ and summing from $t=i$ to $i+\ell-1$,
the additive “shift” terms accumulate only along trajectories that have not yet absorbed,
which contributes the factor $w_t$; let $C\ge C'$ absorb constants and the bound on $w_t\le 1$.
This yields the stated lower bound. The approximation claim follows by dropping $\triangle(s)$,
which is precisely the small conditional-shift term bounded via $\beta_{ok}$. 

This leaves an approximation where the advantage is primarily driven by the reduction in the probability of making a catastrophic error. This proposition is directly supported by the empirical results in Figure-\ref{fig:arm_analyses}, which shows a strong correlation between a module's rank and its per-step error rate.
\end{proof}

\subsection{Theoretical Grounding for the Decoupled Meta-Policy Search}
\label{sec:apdx_meta_policy_theory}
We now justify the zero-shot transfer of a meta-policy $\pi^{\ast}$ discovered using the surrogate $m_{\text{CoT}}$ to the final module $m^{\ast}$. The goal is to show that the expected value of the full system improves, i.e.,
\[
V(\pi^{\ast}(m^{\ast})) \;\geq\; V(\pi^{\ast}(m_{\text{CoT}})).
\]
\begin{proposition}[Module improvement on baseline states]\label{prop:module-improvement}
    The scaffolded meta policy objective optimizes for a module $m^{\ast}$ that has a non-negative expected advantage over the states induced by the baseline policy:
\[
\mathbb{E}_{s \sim d_{m_{\text{CoT}}}}[V_{m^{\ast}}(s)] \;\geq\; \mathbb{E}_{s \sim d_{m_{\text{CoT}}}}[V(s)].
\]
\end{proposition}
\begin{proposition}[Beneficial distribution shift] \label{prop:beneficial-shift}
A superior module $m^{\ast}$, which has a lower error rate on-expectation compared to the baseline (i.e., $\mathbb{E}_{s \sim d_{m_{\text{CoT}}}}[\epsilon_{m^{\ast}}(s)] \leq \mathbb{E}_{s \sim d_{m_{\text{CoT}}}}[\epsilon_{m_{\text{CoT}}}(s)]$), induces a stationary state distribution $d_{m^{\ast}}$ that is weighted towards higher-value states.
\[
\mathbb E_{s\sim d_{m^*}}\big[V_{m^*}(s)\big]\;\ge\;
\mathbb E_{s\sim d_{\text{CoT}}}\big[V_{m^*}(s)\big]
\]
    
\end{proposition}
\begin{itemize}
    \item \textbf{Remark:} Reducing per-step hazard ($S_{fail}$ states) increases expected survival time in $\mathcal S_{ok}$, shifting probability away from $\mathcal S_{fail}$. Since $V_{m^\ast}(s)$ is larger on $\mathcal S_{ok}$ than on $\mathcal S_{fail}$, the expected value under $d_{m^\ast}$ is weakly greater.
\end{itemize}



We now justify the zero-shot transfer of a meta-policy $\pi^*$ discovered using the surrogate $m_{CoT}$ to the final module $m^*$. We aim to show that the expected value of the system improves: $\overline{V}_{m^*} \ge \overline{V}_{m_{CoT}}$. This transfer relies on two premises.
\\
\newtheorem{theorem}{Theorem}

\begin{theorem}[Monotonic Improvement of Meta-Policy Transfer]
Let $\pi(m)$ denote the system using meta-policy $\pi$ and step-generator $m$, and let $V(\pi(m))$ be its expected reward from the initial state distribution. If Proposition~\ref{prop:module-improvement} and Proposition~\ref{prop:beneficial-shift} hold, then the transfer of a meta-policy $\pi^{\ast}$ from $m_{\text{CoT}}$ to $m^{\ast}$ is guaranteed to not degrade performance:
\[
V(\pi^{\ast}(m^{\ast})) \;\geq\; V(\pi^{\ast}(m_{\text{CoT}})).
\]
\end{theorem}
\paragraph{Proof Sketch: } We can decompose the difference in expected values as follows:
\[
V(\pi^{\ast}(m^{\ast})) - V(\pi^{\ast}(m_{\text{CoT}}))
= \mathbb{E}_{s \sim d_{m^{\ast}}}[V_{m^{\ast}}(s)] 
- \mathbb{E}_{s \sim d_{m_{\text{CoT}}}}[V(s)].
\]
We can add and subtract the term  $\mathbb{E}_{s \sim d_{m_{\text{CoT}}}}[V_{m^{\ast}}(s)]$  to obtain:
\[
\begin{aligned}
V(\pi^{\ast}(m^{\ast})) - V(\pi^{\ast}(m_{\text{CoT}}))
&= \underbrace{\Big( 
\mathbb{E}_{s \sim d_{m^{\ast}}}[V_{m^{\ast}}(s)] 
- \mathbb{E}_{s \sim d_{m_{\text{CoT}}}}[V_{m^{\ast}}(s)]
\Big)}_{\text{Gain from Distribution Shift}} \\
&\quad + \underbrace{\Big(
\mathbb{E}_{s \sim d_{m_{\text{CoT}}}}[V_{m^{\ast}}(s)] 
- \mathbb{E}_{s \sim d_{m_{\text{CoT}}}}[V(s)]
\Big)}_{\text{Gain from Module Improvement}}.
\end{aligned}
\]

The first term (\emph{Gain from Distribution Shift}) is non-negative by Proposition-3.  The second term (\emph{Gain from Module Improvement}) is non-negative by Proposition-2.  Since both terms are non-negative, their sum is non-negative, proving the theorem.

This theoretical decomposition is empirically validated by the experiment in Figure~\ref{fig:arm_analyses}.  The performance of \emph{CoT$\to$Meta} relative to \emph{CoT Baseline} measures the Gain from Module Improvement,  while the additional gain seen in the full \emph{Meta Policy} system reflects the Gain from Distribution Shift.  The positive results for both components provide strong empirical support for this theoretical justification.


==> latex/Introduction1.tex <==
\section{Introduction}

Chain-of-thought has been one of the most effective reasoning technique where LLMs reason for a given question over several tokens before arriving at the answer. 

Multi-agent systems (MAS) consist of various LLM agents with defined role, orchestrated via a meta-agent LLM have achieved state-of-the-art results in various complex reasoning tasks. 
With recent advancements in frontier models, especially with reasoning based models, chain-of-thought (CoT) can reason over multiple steps, invoking tools and adaptively/inherently taking on different agent roles at each reasoning step. 
Although MAS approaches achieve SOTA results, recent works have shown that simple CoT outperforms them on various reasoning tasks. Arguably, CoT is one of the earliest technique for solving complex reasoning and it being able to outperform or perform on par with recent complex MAS systems highlights its strength. 
Importantly, majority of the recent progress and efforts have been on development of MAS while CoT baselines have remain fixed. Our work primarily focuses on reshaping CoT in the agentic era by redefining reasoning at each step. 

In this work, we present a sequential reasoning approach named Agentic Reasoning Module (ARM) where each reasoning step is executed by a fundamental reasoning agent A. Motivation behind our work is to enhance thinking steps of CoT from a naive textual reasoning to an agentic block execution. The agentic block in ARM is a generic reasoning procedure that is applied iteratively at each reasoning step. The agentic block is automatically generated by mutation over multiple iterations to perform best on a generic instruction finetuning (IFT) validation data.

Multi-agent systems are highly domain dependent where individual agents are tuned specific to the domain skills. On the other hand, single agent systems are considered to be more generic where reasoning and tool usage are adapted based on the reasoning steps. Nevertheless, even single agent systems are trained for a specific domain or set of tasks. In contrast to all these important directions, our work is focused on redefining or enhancing the prominent CoT reasoning approach with agentic reasoning module. Agent block in our ARM can be tuned over any generic domain resulting in a general reasoning technique same as CoT. We show that our ARM approach outperforms several prominently used MAS approaches on agentic datasets in different domains. Arguably, CoT is one of the earliest technique for solving complex reasoning and it being able to outperform or perform on par with recent complex MAS systems highlights its strength. Importantly, majority of the recent progress and efforts have been on development of MAS while CoT baselines have remain fixed. Our work primarily focuses on reshaping CoT in the agentic era by redefining reasoning at each step. 

CoT, which is one of the most basic, simple yet high performing reasoning approach is used as a starting seed for developing ARM. The meta-agent evolves ARM iteratively via a tree search over the code space, where evolutions are informed by reflection on execution traces. Further, meta-agent discovers global strategies to find best collaborations between parallel ARM reasoning traces to achieve state-of-the-art results, substantially outperforming other MAS systems. Overall, our proposed ARM approach emphasizes on the need of evolving basic and fundamental reasoning methodologies like CoT in contrast to developing more and more complicated heterogeneous MAS systems that are often fragile and need domain tuning.  



\begin{itemize}
    \item We present agentic reasoning module (ARM) which is evolved from CoT. ARM substantially outperforms many of the existing 
    \item We show the ARM is significantly a more generalizable approach compared to previous MAS systems. Thus, highlighting the generalizable nature of ARM for complex reasoning tasks in any domain.
    \item We show detailed ablation analyses of how the performance of ARM improves from each of its components. We show that a concise reflection is essential to improve ARMs. Similarly, global strategy to improve collaboration 
\end{itemize}

% \textcolor{red}{[Shiva - Abstract-V1]}
% Multi-agent systems (MAS) consisting of various LLM agents with defined role, orchestrated via a meta-agent LLM have achieved state-of-the-art results in various complex reasoning tasks. However, manually designing the MAS for various domains requires intensive manual engineering effort and domain knowledge. Thus automatic discovery of MAS has become an emerging field of research with a promise of fully autonomous agents capable of self-orchestration. However, a critical insight is that with frontier models, Chain of Thought (CoT), the fundamental reasoning technique performs competitively with the state-of-the-art MAS approaches. Arguably, CoT is one of the earliest technique for solving complex reasoning and it being able to outperform recent complex MAS systems on frontier models highlights the core hypothesis of our work: the fundamental reasoning process at the heart of each of the agents that constitute any MAS requires some revisiting.

% Multi-agent systems are highly domain dependent where individual agents are tuned specific to the domain skills. On the other hand, single agent systems are considered to be more generic where reasoning and tool usage are adapted based on the reasoning steps. Nevertheless, even single agent systems are trained for a specific domain or set of tasks and focus exclusively on global agent interactions. In contrast to all these important directions, we present a generalized, agentic generalization of CoT for sequential reasoning named Chain of Agent (ARM) where each granular reasoning step is executed by a fundamental reasoning agent. The primary motivation behind our work is to enhance thinking steps of CoT from a naive textual reasoning to an agentic block execution. The agentic block in ARM is a generic reasoning procedure that can applied recursively at each reasoning step. Furthermore, by learning a meta orchestrator (global MAS), the block can be leveraged as a fundamental reasoning primitive within a more complex MAS orchestration. This agentic block is automatically learned by mutation over multiple iterations starting from the fundamental CoT block, and "deep reflection" on the corresponding rollouts. By carefully constructing a scaffolded learning environment, we show that both the recursive application of the block, as well as global orchestration MAS significantly outperform both the manually designed and state-of-the-art MAS approaches. Crucially, our system exhibits strong generalization, maintaining high performance across different foundation models and task domains without modification. 


% \textcolor{red}{[Shiva-Abstract-V2}
% Multi-agent systems (MAS) consisting of various LLM agents with defined role, orchestrated via an LLM meta-agent have achieved state-of-the-art results in various complex reasoning tasks. However, manually designing the MAS for various domains requires intensive manual engineering effort and domain knowledge. Thus automatic discovery of MAS has become an emerging field of research with a promise of fully autonomous agents capable of self-orchestration. However, a critical insight is that with frontier models, Chain of Thought (CoT), the fundamental reasoning technique performs competitively with the state-of-the-art MAS approaches. This observation suggests that the core reasoning mechanism within each agent warrants deeper investigation.


% This work presents a new paradigm for automatic MAS design that pivots the focus to this fundamental reasoning unit. We present an agentic generalization of CoT for sequential reasoning named \textcolor{red}{METHOD NAME} where each granular reasoning step is executed by a reasoning agent. The primary motivation behind our work is to enhance thinking steps of CoT from a naive textual reasoning to an agentic block execution. The agentic block acts as a versatile, generic reasoning procedure that can be leveraged within a more complex MAS . We demonstrate it's effectiveness through two deployment strategies: first, as a direct zero-shot recursive loop, and secondly as a subroutine in a learned meta orchestrator. The agentic block is discovered through an iterative search over the code space, guided by Thompson Sampling. Starting from a foundational Chain-of-Thought (CoT) block, this process uses mutations informed by deep reflection on execution rollouts to progressively refine the agent's code. By carefully constructing a scaffolded learning environment, we show that both the recursive application of the block, as well as learned orchestration MAS significantly outperform both the manually designed and state-of-the-art MAS approaches. Crucially, our system exhibits strong generalization, maintaining high performance across different foundation models and task domains without modification. 

